Pileup density estimate independent on jet multiplicity

The hard-scatter processes in hadronic collisions are often largely contaminated with soft background coming from pileup in proton-proton collisions, or underlying event in heavy-ion collisions. There are multiple methods to remove the effect of pileup for jets. Two such methods, Area Subtraction and Constituent Subtraction, use the pileup density as the main ingredient to estimate the magnitude of pileup contribution on an event-by-event basis. The state-of-the-art approaches to estimating pileup density are sensitive to the number of hard-scatter jets in the event. This paper presents a new pileup-density estimation method that minimizes the sensitivity on the presence of hard-scatter jets in the event. Using a detector-level simulation, we provide a comparison of the new method with the state-of-the-art estimation methods. We observe a significantly lower bias for the estimated pileup density when using the new method. We conclude that the new method has the potential to significantly improve pileup mitigation in proton-proton collisions or the underlying event subtraction in heavy-ion collisions.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = ms

default: dopdflatexwithbibtex


dopdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	make clean

dopdflatexwithbibtex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	make clean


clean:
	rm -f *.aux *.log *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~  spellTmp ${BASENAME}.ps



==> defs.tex <==
%
% User-defined latex commands
%
\RequirePackage{xspace}

\newcommand{\mname}{\texttt{SignalFreeBackgroundEstimator}}


\newcommand{\tev}               {\ensuremath{~\mathrm{TeV}}\xspace}
\newcommand{\gev}               {\ensuremath{~\mathrm{GeV}}\xspace}
\newcommand{\mev}               {\ensuremath{~\mathrm{MeV}}\xspace}

% Jet mass related
\newcommand{\mjet}               {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\mlead}              {\ensuremath{\mjet_{1}}\xspace}
\newcommand{\mleadavg}           {\ensuremath{\langle\mlead\rangle}\xspace}
\newcommand{\Mjet}               {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\massjet}            {\mjet}
\newcommand{\mjetAvg}            {\ensuremath{\langle\mjet\rangle}\xspace}
\newcommand{\masstrkjet}         {\ensuremath{m^{\rm track \; jet}}\xspace}

% Particle (and mass) related
\newcommand{\Wmass}              {\ensuremath{m_{\Wboson}}\xspace}
\newcommand{\WmassT}             {\ensuremath{m^{\Wboson}_{\rm T}}\xspace}
\newcommand{\topmass}            {\ensuremath{m_{t}}\xspace}
\newcommand{\mTransv}            {\ensuremath{m_{\rm T}}\xspace}
\newcommand{\massZprime}         {\ensuremath{m_{\Zprime}}\xspace}

% Jet algorithm and grooming related
\newcommand{\antikt}             {anti-\ensuremath{k_{t}}\xspace}
\newcommand{\akt}                {\antikt\xspace}
\newcommand{\aktfour}            {\antikt \ensuremath{R=0.4}\xspace}
\newcommand{\aktten}            {\antikt \ensuremath{R=1.0}\xspace}
\newcommand{\kt}                 {\ensuremath{k_{t}}\xspace}
\newcommand{\ca}                 {Cambridge--Aachen\xspace}
\newcommand{\CamKt}              {\ensuremath{\mathrm{C/A}}\xspace}
\newcommand{\CASix}              {\CamKt, \ensuremath{R=0.6}\xspace}
\newcommand{\CAFat}              {\CamKt, \ensuremath{R=1.2}\xspace}
\newcommand{\CAPrune}            {\CamKt, \ensuremath{R=1.2} (pruned)\xspace}
\newcommand{\CAFilt}             {\CamKt, \ensuremath{R=1.2} (filtered)\xspace}
\newcommand{\SISCone}            {SISCone}
\newcommand{\SISConeSiz}         {\SISCone, \ensuremath{R=0.6}\xspace}
\newcommand{\minKt}              {\ensuremath{\min\left(\pti^2, \ptj^2\right)}\xspace}
\newcommand{\minAKt}             {\ensuremath{\min\left(\pti^{-2}, \ptj^{-2}\right)}\xspace}
\newcommand{\minGen}             {\ensuremath{\min\left(\pti^{2p}, \ptj^{2p}\right)}\xspace}
\newcommand{\pt}                 {\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand{\et}                 {\ensuremath{E_{\mathrm{T}}}\xspace}
\newcommand{\etmiss}             {\ensuremath{E_{\mathrm{T}}^{\mathrm{miss}}}\xspace}
\newcommand{\etmissx}            {\ensuremath{E_{\mathrm{T},x}^{\mathrm{miss}}}\xspace}
\newcommand{\etmissVec}          {\ensuremath{\vec{E}_{\mathrm{T}}^{\mathrm{miss}}}\xspace}
\newcommand{\pttrue}             {\ensuremath{\pt^{\mathrm{true}}}\xspace}
\newcommand{\ptreco}             {\ensuremath{\pt^{\mathrm{reco}}}\xspace}
\newcommand{\Rij}                {\ensuremath{R_{ij}}\xspace}
\newcommand{\DRij}               {\ensuremath{\Delta\Rij}\xspace}
\newcommand{\DRratio}            {\ensuremath{\frac{(\DRij)^2}{R^2}}\xspace}
\newcommand{\sjone}              {\ensuremath{j_{1}}\xspace}
\newcommand{\sjtwo}              {\ensuremath{j_{2}}\xspace}
\newcommand{\msubjone}           {\ensuremath{m^{\sjone}}\xspace}
\newcommand{\msubjtwo}           {\ensuremath{m^{\sjtwo}}\xspace}
\newcommand{\ptsubjone}          {\ensuremath{\pt^{\sjone}}\xspace}
\newcommand{\ptsubjtwo}          {\ensuremath{\pt^{\sjtwo}}\xspace}
\newcommand{\Rsubjets}           {\ensuremath{R_{\sjone,\sjtwo}}\xspace}
\newcommand{\DRsubjets}          {\ensuremath{\Delta\Rsubjets}\xspace}
\newcommand{\Nsubjet}            {\ensuremath{N_{\rm subjet}}\xspace}
\newcommand{\pti}                {\ensuremath{p_{\mathrm{T},i}}\xspace}
\newcommand{\pticorr}            {\ensuremath{\pti^{\rm corr}}\xspace}
\newcommand{\ptpatch}            {\ensuremath{p_{{\rm T patch}}}\xspace}
\newcommand{\ptpatchi}            {\ensuremath{p^{\rm patch}_{T,i}}\xspace}
\newcommand{\ptj}                {\ensuremath{p_{{\rm T}j}}\xspace}
\newcommand{\phii}               {\ensuremath{\phi_{i}}\xspace}
\newcommand{\yi}                 {\ensuremath{y_{i}}\xspace}
\newcommand{\mi}                 {\ensuremath{m_{i}}\xspace}
\newcommand{\mdelta}             {\ensuremath{m_{\delta}}\xspace}
\newcommand{\mdeltai}            {\ensuremath{m_{\delta i}}\xspace}
\newcommand{\mdeltapatch}        {\ensuremath{m_{\delta \rm patch}}\xspace}
\newcommand{\mdeltaicorr}        {\ensuremath{\mdeltai^{\rm corr}}\xspace}
\newcommand{\ycut}               {\ensuremath{y_{\rm cut}}\xspace}
\newcommand{\mcut}               {\ensuremath{m_{\rm cut}}\xspace}
\newcommand{\ymin}               {\ensuremath{y_{\min}}\xspace}
\newcommand{\fcut}               {\ensuremath{f_{\rm cut}}\xspace}
\newcommand{\Rsub}               {\ensuremath{R_{\rm sub}}\xspace}
\newcommand{\drsub}              {\ensuremath{\Rsub}\xspace}
\newcommand{\mufrac}             {\ensuremath{\mu_{\rm frac}}\xspace}
\newcommand{\rcut}               {\ensuremath{R_{\rm cut}}\xspace}
\newcommand{\zcut}               {\ensuremath{z_{\rm cut}}\xspace}
\newcommand{\largeR}             {large-\ensuremath{R}\xspace}
\newcommand{\LargeR}             {Large-\ensuremath{R}\xspace}


% Jet substructure related
\newcommand{\shapeV}             {\ensuremath{{\cal V}}\xspace}
\newcommand{\htt}                {HEPTopTagger\xspace}
\newcommand{\subjetpt}           {\ensuremath{\pT^{\rm subjet}}\xspace}
\newcommand{\subjetptl}          {\ensuremath{\pT^{\rm subjet, lead}}\xspace}
\newcommand{\subjetptsl}         {\ensuremath{\pT^{\rm subjet, sublead}}\xspace}
\newcommand{\yij}                {\ensuremath{y_{ij}}\xspace}
\newcommand{\dcut}               {\ensuremath{d_{\rm cut}}\xspace}
\newcommand{\dmin}               {\ensuremath{d_{\min}}\xspace}
\newcommand{\dij}                {\ensuremath{d_{ij}}\xspace}
\newcommand{\Dij}                {\ensuremath{\sqrt{\dij}}\xspace}
\newcommand{\DOneTwo}            {\ensuremath{\sqrt{d_{12}}}\xspace}
\newcommand{\DTwoThr}            {\ensuremath{\sqrt{d_{23}}}\xspace}
\newcommand{\xj}                 {\ensuremath{x_{J}}\xspace}
\newcommand{\jetFunc}            {\ensuremath{J^{(eik),c} (\mjet, \pT, R)}\xspace}
\newcommand{\tauN}               {\ensuremath{\tau_N}\xspace}
\newcommand{\tauOne}             {\ensuremath{\tau_{1}}\xspace}
\newcommand{\tauTwo}             {\ensuremath{\tau_{2}}\xspace}
\newcommand{\tauThr}             {\ensuremath{\tau_{3}}\xspace}
\newcommand{\tauTwoOne}          {\ensuremath{\tau_{21}}\xspace}
\newcommand{\tauThrTwo}          {\ensuremath{\tau_{32}}\xspace}
\newcommand{\COneThr}            {\ensuremath{C_{1}^{(3)}}\xspace}

% Samples
\newcommand{\ttbar}           {\ensuremath{t\bar{t}}\xspace}
\newcommand{\tttt}           {\ensuremath{t\bar{t}t\bar{t}}\xspace}
\newcommand{\Zprimett}           {\ensuremath{Z'\ra t\bar{t}}\xspace}
\newcommand{\Zprime}             {\ensuremath{Z'}\xspace}
\newcommand{\Zqq}                {\ensuremath{Z\ra q\bar{q}}\xspace}
\newcommand{\Wqq}                {\ensuremath{W\ra q\bar{q}}\xspace}


% terminology
\newcommand{\mpi}                {multiple parton interactions\xspace}
\newcommand{\fourvector}         {4-vector\xspace}
\newcommand{\fourmomentum}       {4-momentum\xspace}
\newcommand{\fourmomenta}        {4-momenta\xspace}
\newcommand{\pileup}             {pileup\xspace}
\newcommand{\Pileup}             {Pileup\xspace}
\newcommand{\areaSubtraction}    {Area Subtraction\xspace}
\newcommand{\cs}        {Constituent Subtraction\xspace}
\newcommand{\ics}                {Iterative Constituent Subtraction\xspace}


       
\newcommand{\avg}[1]             {\left< #1 \right>} % e.g. <\mu>

% rho estimation related
\newcommand{\rhom}               {\ensuremath{\rho_{m}}\xspace}
\newcommand{\rhoest}             {\ensuremath{\rho_{\mathrm{est}}}\xspace}
\newcommand{\rhotrue}            {\ensuremath{\rho_{\mathrm{true}}}\xspace}
\newcommand{\Rexclude}           {\ensuremath{R_{\mathrm{exclude}}}\xspace}
\newcommand{\Smin}               {\ensuremath{S_{\mathrm{max}}}\xspace}

\newcommand{\Rmin}               {\ensuremath{R_{\rm min}}}
\newcommand{\DeltaR}             {\ensuremath{\Delta R}\xspace}
\newcommand{\DeltaRhard}         {\ensuremath{\Delta R^{\mathrm{hard}}}\xspace}
\newcommand{\DeltaRmax}          {\ensuremath{\Delta R^{\mathrm{max}}}\xspace}
\newcommand{\DeltaRik}           {\ensuremath{\Delta R_{i,k}}\xspace}
\newcommand{\Dik}                {\ensuremath{D_{i,k}}\xspace}
\newcommand{\Dy}                 {\ensuremath{\Delta y}\xspace}
\newcommand{\Deta}               {\ensuremath{\Delta\eta}\xspace}
\newcommand{\Dphi}               {\ensuremath{\Delta\phi}\xspace}
\newcommand{\maxEta}             {\ensuremath{\eta^{\mathrm{max}}}\xspace}


% pileup subtraction related
\newcommand{\ptInput}            {\ensuremath{\pt^{\mathrm{input}}}\xspace}
\newcommand{\ptOutput}           {\ensuremath{\pt^{\mathrm{output}}}\xspace}
\newcommand{\ghostpt}            {\ensuremath{\pt^g}\xspace}
\newcommand{\ghostptk}           {\ensuremath{p_{{\rm T}k}^g}\xspace}
\newcommand{\ghostptkSquared}    {\ensuremath{p_{{\rm T}k}^{g2}}\xspace}
\newcommand{\ghostphik}          {\ensuremath{\phi_{k}^g}\xspace}
\newcommand{\ghostyk}            {\ensuremath{y_{k}^g}\xspace}
\newcommand{\ghostm}             {\ensuremath{m^g}\xspace}
\newcommand{\ghostmk}            {\ensuremath{m_{k}^g}\xspace}
\newcommand{\ghostmkSquared}     {\ensuremath{m_{k}^{g2}}\xspace}
\newcommand{\ghostmdelta}        {\ensuremath{m_{\delta}^g}\xspace}
\newcommand{\ghostmdeltak}       {\ensuremath{m_{\delta k}^g}\xspace}
\newcommand{\ghostptavg}         {\ensuremath{\langle\ghostpt\rangle}\xspace}
\newcommand{\ghostfm}            {\ensuremath{g_{\mu}}\xspace}
\newcommand{\ghostfmi}           {\ensuremath{g_{\mu,i}}\xspace}
\newcommand{\ghostdensity}       {\ensuremath{\nu_{g}}\xspace}
\newcommand{\ghostrho}           {\ensuremath{\ghostdensity\ghostptavg}\xspace}
\newcommand{\Aghost}             {\ensuremath{A_{g}}\xspace}
\newcommand{\Amu}                {\ensuremath{A_{\mu}}}
\newcommand{\Amui}               {\ensuremath{A_{\mu, i}}}
\newcommand{\jetarea}            {\ensuremath{A^{\mathrm{jet}}}\xspace}
\newcommand{\jetareafm}          {\ensuremath{A^{\mathrm{jet}}_{\mu}}\xspace}
\newcommand{\jetareai}           {\ensuremath{\jetarea_{i}}\xspace}
\newcommand{\areapatch}          {\ensuremath{A_{\rm patch}}\xspace}
\newcommand{\areapatchi}          {\ensuremath{A^{\rm patch}_i}\xspace}
\newcommand{\rkt}                {\ensuremath{R_{\kt}}\xspace}
\newcommand{\yphi}                {\ensuremath{y -\phi}\xspace}
\newcommand{\etaphi}                {\ensuremath{\eta -\phi}\xspace}

\newcommand{\ptorig}             {\ensuremath{p_T^{\rm orig}}\xspace}
\newcommand{\npu}                {\ensuremath{N_{PU}}\xspace}
\newcommand{\avgnpu}             {\ensuremath{\avg{\npu}}\xspace}
\newcommand{\avgrho}             {\ensuremath{\avg{\rho}}\xspace}
\newcommand{\sigmarho}           {\ensuremath{\sigma[\rho]}\xspace}
\newcommand{\Niter}           {\ensuremath{N^{\mathrm{iter}}}\xspace}



\newcommand{\meanDelta}          {\ensuremath{\langle \Delta x \rangle}\xspace}
\newcommand{\sigmaDelta}         {\ensuremath{\sigma[\Delta x]}\xspace}
\newcommand{\ptSum}         {\ensuremath{\langle\sum \pt\rangle}\xspace}
\newcommand{\ptSumTrue}         {\ensuremath{\langle\sum \pt^{\mathrm{true}}\rangle}\xspace}

